DualDiff: Dual-branch Diffusion Model for Autonomous Driving with Semantic Fusion

Accurate and high-fidelity driving scene reconstruction relies on fully leveraging scene information as conditioning. However, existing approaches, which primarily use 3D bounding boxes and binary maps for foreground and background control, fall short in capturing the complexity of the scene and integrating multi-modal information. In this paper, we propose DualDiff, a dual-branch conditional diffusion model designed to enhance multi-view driving scene generation. We introduce Occupancy Ray Sampling (ORS), a semantic-rich 3D representation, alongside numerical driving scene representation, for comprehensive foreground and background control. To improve cross-modal information integration, we propose a Semantic Fusion Attention (SFA) mechanism that aligns and fuses features across modalities. Furthermore, we design a foreground-aware masked (FGM) loss to enhance the generation of tiny objects. DualDiff achieves state-of-the-art performance in FID score, as well as consistently better results in downstream BEV segmentation and 3D object detection tasks.

==> sections/1.intro_old.tex <==
\section{Introduction}
Most vision-based research solutions in autonomous driving today rely heavily on large-scale datasets collected via cameras, along with detailed annotations \cite{cui2024survey}, \cite{MARTINEZDIAZ2018275}, \cite{chen2024end}. However, due to the high costs of real-world data collection and annotation, the availability of open-source autonomous driving vision datasets remains limited \cite{BOSCH201876}, \cite{10432820}. Therefore, diffusion models based on Stable Diffusion \cite{rombach2022high}, \cite{li2023drivingdiffusion}, \cite{song2020denoising} have achieved remarkable breakthroughs in generating realistic images, providing a feasible approach for synthesizing street-view data. 

% Previous works\cite{wen2024panacea},\cite{gao2023magicdrive},\cite{zhang2024perldiff} project driving scene maps into camera-view or bird's-eye-view (BEV), with foreground elements like 3D bounding boxes projected into camera-view or treated as sequence with variable length. These methods also use text prompts to control contextual semantic information such as weather and lighting conditions. Drive-WM\cite{wang2024drivewm} extends driving scene reconstruction to video generation, utilizing Unified Conditions consisting of text prompts, boxes, and maps as environmental control signals, injected into the cross-attention modules of the Unet\cite{ronneberger2015u}. DriveDreamer-2\cite{zhao2024drivedreamer2} employs an additional diffusion model to generate BEV maps based on user-specified trajectories, combined with camera-view projected bounding boxes for scene reconstruction.
% Conditional generation networks, such as ControlNet \cite{zhang2023controlnet}, effectively utilizes semantic segmentation maps, sketches, or other types of inputs as conditions to precisely control the content of generated images. This provides a promising direction for editable street-view image generation. In the field of autonomous driving, previous works \cite{wen2024panacea} \cite{gao2023magicdrive} project driving scene maps into camera-view or bird's-eye-view (BEV), with foreground elements like 3D bounding boxes projected into camera-view or treated as sequence with variable length. These methods also use text prompts to control contextual semantic information such as weather and lighting conditions. Drive-WM \cite{wang2024drivewm} extends driving scene reconstruction to video generation, utilizing Unified Conditions consisting of text prompts, boxes, and maps as environmental control signals, injected into the cross-attention modules of the Unet. DriveDreamer-2 \cite{zhao2024drivedreamer2} employs an additional diffusion model to generate BEV maps based on user-specified trajectories, combined with camera-view projected bounding boxes for scene reconstruction.

% Many of these models have successfully generated high-fidelity driving street views, serving as data supplementation or augmentation for downstream vision-based tasks. However, none of the previous works have explored the effective integration of semantic 3D scene information such as semantic point clouds or occupancy (occ) voxels. These types of data provide comprehensive scene characteristics, including the outlines and relative positions of foreground entities, the overall layout and detailed shapes of the background, and even novel instances like building blocks that are not included in bounding boxes or map mask annotations. 
\begin{figure}
\centering{}
\includegraphics[width=0.9\linewidth]{figs/lidar3.png}
\caption{We have achieved state-of-the-art performance in several evaluation metrics compared to other custom or base models. To present the data in the charts more clearly, we have scaled some of the metrics.} \label{fig: lidar}
\vspace{-0.6cm}
\end{figure}
Many of these methods have successfully generated high-fidelity driving street scenes, providing data supplementation or enhancement for downstream visual tasks. However, no previous studies have explored the effective integration of rich semantic 3D scene information such as semantic point clouds or occupied voxels. These types of data are very important. They provide rich full-scene features, including the outlines and relative positions of foreground entities, the overall layout and detailed shapes of the background, and even new instances such as building blocks that are not included in the bounding box or map mask annotations. 
% Thus, this paper focuses on the task of scene reconstruction based on 3D semantic representations in autonomous driving, introducing two modalities of scene information: occ-based scene representations and numerical scene representations. We propose an innovative dual-branch foreground-background architecture to exert detailed control over the generation process. Furthermore, we introduce a Semantic Fusion Attention module (SFA) to establish connections and interactions between the input multi-modal scene information, further enhancing the model’s scene understanding.

Therefore, our focus is on studying the scene reconstruction task with efficient fusion of 3D semantic information in autonomous driving. We innovatively propose a \textbf{decoupled dual-branch} (foreground-background) structure and establish connections and interactions between multi-modal input scene information based on the proposed \textbf{semantic fusion attention module} (SFA), further enhancing the scene understanding of the model. {To address the existing challenge of tiny objects, we further explore the available 3D box information and design a simple yet effective \textbf{foreground-aware masked} (FGM) loss.} {Specially, we use the camera view projected box to construct a weighted mask for the original denoising loss in order to focus more on regions belonging to tiny objects.}

% 前景背景生成表现不一致：在自动驾驶场景生成中，前景和背景包含不同类型的细节和特征，需要分别处理以实现高质量的场景重建。然而，传统方法使用的信息模态较为有限，无法充分表征复杂的驾驶场景，导致生成效果在兼顾前景和背景细节方面表现不佳。

% 多模态信息整合不足：在自动驾驶场景生成中，多模态输入（如相机视角、地图数据和边界框）包含了不同类型的信息，这些信息需要有效协调和融合以提高生成模型的场景理解和重建精度。现有的方法往往难以有效地整合这些多模态信息，导致生成效果无法全面反映场景的复杂性。
% 微小物体细节的强化不足：在自动驾驶场景生成中，如何处理和强化微小物体的细节是一个关键。现有的生成模型往往难以准确捕捉这些微小物体，导致它们在生成结果中被忽视或细节不充分。然而，这些微小物体在实际应用中非常重要，因为它们对场景的整体准确性和可靠性具有关键影响。
Our proposed model effectively integrates cross-modal scene features, enabling the accurate reconstruction of scene content, and outperforms previous methods in terms of image style fidelity, foreground attributes, and background layout accuracy. The main contributions of this work are summarized below.
\begin{itemize}
\item We first propose a decoupled dual-branch (foreground-background) architecture that leverages our introduced occupancy ray sampling (ORS) representation and numerical driving scene representation, to exert fully control upon the scene reconstruction process.
% 我们首次提出了一种解耦的双分支（前景-背景）架构，该架构利用了基于体素的场景表示和数字场景表示，全面掌控场景重建过程。这种双分支结构使得前景和背景可以分别进行优化，进而实现对复杂场景的精确控制，确保了生成结果的高保真度和细节丰富性。
\item
% The introduction of the Semantic Fusion Attention module allows for the efficient fusion and interaction of the multi-modal environmental information input to the model, improving its scene understanding capabilities.
We propose an efficient semantic fusion attention (SFA) module to improve the understanding of multi-modal scene representations. In addition, we propose a foreground-aware masked (FGM) Loss to further improve the generation of tiny objects.
\item 
% During the model training phase, we design a ForeGround-aware Masked loss (FGM loss) upon the original diffusion denoising loss to further enhance the generation of tiny objects. Our model outperforms previous best methods in its ability to reconstruct realistic styles and accurately generate foreground and background content, achieving state-of-the-art performance.
Our model surpasses the previous best methods in terms of realistic style reconstruction and accurate generation of foreground and background content, achieving the state-of-the-art (SOTA) performance.
\end{itemize}





==> tables/bevfusion_and_cvt.tex <==
% \begin{table}
% \centering{}%
% \scalebox{0.96}{
% \begin{tabular}{c|c|c|c|c}
% \toprule
% Data & mAP $\uparrow$ & mAOE $\downarrow$ & mAVE $\downarrow$ & NDS $\uparrow$ \\
% \midrule

%    w/o synthetic data & 34.5 & 59.4 & 29.1 & 46.9 \\

%    w/ PanaCea\cite{wen2024panacea}
%    & \textbf{37.1 {\tiny\textcolor{green}{+2.6\%}}}
%    & 54.2\textbf{ {\tiny\textcolor{red}{-5.2\%}}}
%    & \textbf{27.3 {\tiny\textcolor{red}{-1.8\%}}}
%    & \textbf{49.2 {\tiny\textcolor{green}{+2.3\%}}}
%    \\

%    w/ Ours
%    & 35.9\textbf{ {\tiny\textcolor{green}{+1.4\%}}}
%    & \textbf{50.9 {\tiny\textcolor{red}{-8.5\%}}}
%    & 29.8\textbf{ {\tiny\textcolor{green}{+0.7\%}}}
%    & 49.1\textbf{ {\tiny\textcolor{green}{+2.2\%}}}
%    \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparison about support training for 3D object detection model (StreamPETR \cite{wang2023streampetr}). Results are reported on the nuScenes validation set.}
% \vspace{-0.6cm}
% \label{tab:streampetr_train}
% \end{table}

% \begin{table}
% \centering{}%
% \scalebox{0.84}{
% \begin{tabular}{ccc|ccc}
% \toprule
% Dual Branch & SFA & FGM Loss & FID$\downarrow$ & Road mIoU$\uparrow$ & Vehicle mIoU$\uparrow$ \\% & mAP $\uparrow$ & mAOE $\downarrow$ & NDS $\uparrow$ \\ %mAVE $\downarrow$ & 
% \midrule

% & & & 13.26 & 62.19 & 27.30 \\%11.39 & 78.07 & 22.88 \\  % & 110.85
% & & \checkmark & 12.95 & 61.78 & 29.00 \\%13.56 & 69.72 & 25.05 \\ % & 112.55
% &  \checkmark & \checkmark & 12.57 & 61.47 & 29.11 \\%13.84 & 71.22 & 24.76 \\ % & 105.82
% \checkmark & \checkmark & & {11.01} & {62.71} & {29.19} \\
% \checkmark & \checkmark & \checkmark & \textbf{10.99} & \textbf{62.75} & \textbf{30.22} \\
   
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation studies on proposed modules with respect to FID score and downstream BEV segmentation task (CVT).}
% \vspace{-0.6cm}
% \label{tab:ablation}
% \end{table}
